When is BERT Multilingual? Isolating Crucial Ingredients for Cross-lingual Transfer

While recent work on multilingual language models has demonstrated their capacity for cross-lingual zero-shot transfer on downstream tasks, there is a lack of consensus in the community as to what shared properties between languages enable such transfer. Analyses involving pairs of natural languages are often inconclusive and contradictory since languages simultaneously differ in many linguistic aspects. In this paper, we perform a large-scale empirical study to isolate the effects of various linguistic properties by measuring zero-shot transfer between four diverse natural languages and their counterparts constructed by modifying aspects such as the script, word order, and syntax. Among other things, our experiments show that the absence of sub-word overlap significantly affects zero-shot transfer when languages differ in their word order, and there is a strong correlation between transfer performance and word embedding alignment between languages (e.g., R=0.94 on the task of NLI). Our results call for focus in multilingual models on explicitly improving word embedding alignment between languages rather than relying on its implicit emergence.

==> OldTables/JointTable.tex <==
\begin{table*}[t]
\centering
% Uncomment to resize
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccccc}\toprule
% Header -------------------------------------
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Language}} & \multicolumn{3}{c}{\textbf{Inversion}} & \multicolumn{3}{c}{\textbf{Permutation}} & \multicolumn{3}{c}{\textbf{Syntax}} & \multicolumn{3}{c}{\textbf{Transliteration}}\\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 

 & & \zs & \supdiff & \monodiff & \zs & \supdiff & \monodiff & \zs & \supdiff & \monodiff & \zs & \supdiff & \monodiff\\ \midrule

% Template
% English & 73.2 & -2.5  & 11.5 & 68.6 & -7.5  & 2.7 & 61.2 & -13.7 & -0.8 & 74.1 & -2.1 & 40.8 & 33.5 & -41   & 0 \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% XNLI %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{\textbf{XNLI}} & \textbf{English} & 73.2 & \ApplyGradient{-3.4} & \ApplyGradient{11.5} & 68.6 & \ApplyGradient{-5} & \ApplyGradient{2.7} & 74.1 & \ApplyGradient{-1.8} & \ApplyGradient{-0.3} & 74.1 & \ApplyGradient{-1.7} & \ApplyGradient{40.8}\\
& \textbf{French} & 62.5 & \ApplyGradient{-9.5} & \ApplyGradient{-0.7} & 68.4 & \ApplyGradient{-1} & \ApplyGradient{6.6} & 69.6 & \ApplyGradient{-2.2} & \ApplyGradient{-0.8} & 71.6 & \ApplyGradient{-1.6} & \ApplyGradient{38.3}\\
& \textbf{Hindi} & 43.9 & \ApplyGradient{-15.7} & \ApplyGradient{0.1} & 51.2 & \ApplyGradient{-6.2} & \ApplyGradient{6.9} & 61.6 & \ApplyGradient{-0.3} & \ApplyGradient{1.3} & 63.4 & \ApplyGradient{-0.1} & \ApplyGradient{29.3}\\
& \textbf{Arabic} & 54 & \ApplyGradient{-12.3} & \ApplyGradient{0.2} & 62.1 & \ApplyGradient{-2.3} & \ApplyGradient{3.7} & 65.9 & \ApplyGradient{0.7} & \ApplyGradient{0.4} & 68 & \ApplyGradient{-0.4} & \ApplyGradient{34.7} \\ \cdashlinelr{1-14}
& \textbf{Avg.} &  & \textbf{\ApplyGradient{-10.2}} & \textbf{\ApplyGradient{2.8}} &  & \textbf{\ApplyGradient{-3.6}} & \textbf{\ApplyGradient{5.0}} &  & \textbf{\ApplyGradient{-0.9}} & \textbf{\ApplyGradient{0.2}} &  & \textbf{\ApplyGradient{-1.0}} & \textbf{\ApplyGradient{35.8}} \\ \midrule
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NER %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{\textbf{NER}} & \textbf{English} & 39.8 & \ApplyGradient{-44.5} & \ApplyGradient{-8.6} & 40.2 & \ApplyGradient{-28.5} & \ApplyGradient{4.7} & 61.1 & \ApplyGradient{-7.8} & \ApplyGradient{2.5} & 78 & \ApplyGradient{-2.1} & \ApplyGradient{68.1} \\
& \textbf{French} & 54.5 & \ApplyGradient{-34.4} & \ApplyGradient{16.9} & 44.4 & \ApplyGradient{-36.0} & \ApplyGradient{3.8} & 59.6 & \ApplyGradient{-21.9} & \ApplyGradient{4} & 84.3 & \ApplyGradient{-3.1} & \ApplyGradient{84.3} \\
& \textbf{Hindi} & 19.4 & \ApplyGradient{-63.9} & \ApplyGradient{-0.7} & 38.5 & \ApplyGradient{-21.9} & \ApplyGradient{15.5} & 64.8 & \ApplyGradient{-8.4} & \ApplyGradient{-1.1} & 84.4 & \ApplyGradient{-0.5} & \ApplyGradient{82.4} \\
& \textbf{Arabic} & 37.8 & \ApplyGradient{-53.6} & \ApplyGradient{-17.3} & 66.2 & \ApplyGradient{-18.8} & \ApplyGradient{12.3} & 66.1 & \ApplyGradient{-20.1} & \ApplyGradient{2.9} & 88 & \ApplyGradient{-1.9} & \ApplyGradient{88} \\  \cdashlinelr{1-14}
& \textbf{Avg.} &  & \textbf{\ApplyGradient{-49.1}} & \textbf{\ApplyGradient{-2.4}} &  & \textbf{\ApplyGradient{-26.3}} & \textbf{\ApplyGradient{9.1}} &  & \textbf{\ApplyGradient{-14.6}} & \textbf{\ApplyGradient{2.1}} &  & \textbf{\ApplyGradient{-1.9}} & \textbf{\ApplyGradient{80.7}} \\ \midrule
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% POS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{\textbf{POS}} & \textbf{English} & 94.4 & \ApplyGradient{-0.7} & \ApplyGradient{23.6} & 78.3 & \ApplyGradient{-11.9} & \ApplyGradient{5.7} & 92.9 & \ApplyGradient{-0.9} & \ApplyGradient{1.3} & 94.6 & \ApplyGradient{-0.5} & \ApplyGradient{94.6}\\
& \textbf{French} & 74.3 & \ApplyGradient{-22.7} & \ApplyGradient{0.2} & 82 & \ApplyGradient{-12.2} & \ApplyGradient{8.7} & 93.5 & \ApplyGradient{-3.2} & \ApplyGradient{2} & 97.2 & \ApplyGradient{-0.2} & \ApplyGradient{97.2}\\
& \textbf{Hindi} & 19 & \ApplyGradient{-74.5} & \ApplyGradient{0} & 51 & \ApplyGradient{-14} & \ApplyGradient{27.8} & 91.6 & \ApplyGradient{-3.3} & \ApplyGradient{8} & 96.5 & \ApplyGradient{-0.1} & \ApplyGradient{96.5} \\
& \textbf{Arabic} & 69.2 & \ApplyGradient{-23.0} & \ApplyGradient{0} & 83.1 & \ApplyGradient{-6.5} & \ApplyGradient{14.1} & 79.4 & \ApplyGradient{-10} & \ApplyGradient{1.5} & 93.2 & \ApplyGradient{-0.8} & \ApplyGradient{90.1} \\ \cdashlinelr{1-14}
& \textbf{Avg.} &  & \textbf{\ApplyGradient{-30.2}} & \textbf{\ApplyGradient{6.0}} &  & \textbf{\ApplyGradient{-11.2}} & \textbf{\ApplyGradient{14.1}} &  & \textbf{\ApplyGradient{-4.4}} & \textbf{\ApplyGradient{3.2}} &  & \textbf{\ApplyGradient{-0.4}} & \textbf{\ApplyGradient{94.6}} \\ \midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% XQuAD %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{\textbf{XQuAD}} & \textbf{English} & 30.4 & \ApplyGradient{-43.2} & \ApplyGradient{-7.7} & - & - & - & - & - & - & 72.4 & \ApplyGradient{-4} & \ApplyGradient{69} \\
& \textbf{French} & 25.2 & \ApplyGradient{-29.5} & \ApplyGradient{0.1} & - & - & - & - & - & - & 60.9 & \ApplyGradient{-1} & \ApplyGradient{54.5} \\
& \textbf{Hindi} & 14.5 & \ApplyGradient{-27.3} & \ApplyGradient{0} & - & - & - & - & - & - & 57.3 & \ApplyGradient{10.6} & \ApplyGradient{54.1} \\
& \textbf{Arabic} & 21 & \ApplyGradient{-31.2} & \ApplyGradient{0.2} & - & - & - & - & - & - & 54 & \ApplyGradient{-0.5} & \ApplyGradient{51.2} \\ \cdashlinelr{1-14}
& \textbf{Avg.} &  & \textbf{\ApplyGradient{-32.8}} & \textbf{\ApplyGradient{-1.9}} &  &  &  &  &  &  &  & \textbf{\ApplyGradient{1.3}} & \textbf{\ApplyGradient{57.2}}\\

\bottomrule
\end{tabular}
% Uncomment to resize resize
}
\caption{New joint table which will replace the two tables we currently have. \todo{Make the averages look more prominent.}\label{table:joint_table}}
\end{table*}

==> Tables/ComposedTrans.tex <==
\begin{table}[t]
\centering
% Uncomment to resize
% \resizebox{\linewidth}{!}{
\begin{tabular}{cccc}\toprule
% Header -------------------------------------

%  \multirow{2}{*}{\textbf{Transformation}} & \multicolumn{2}{c}{\textbf{XNLI}} & \multicolumn{2}{c}{\textbf{NER}} & \multicolumn{2}{c}{\textbf{POS}} \\
\multirow{2}{*}{\textbf{Transformation}} & \multicolumn{3}{c}{\supdiff} \\
\cmidrule(lr){2-4}
  & \textbf{XNLI} & \textbf{NER} & \textbf{POS} \\ \midrule
  \textbf{Transliteration} & -1.7 & -2.1 & -0.5 \\ \cdashlinelr{1-4}
  \textbf{Inversion} & -3.4 & -44.5 & -0.7 \\
 \textbf{Trans. $\circ$ Inv.} & \cellcolor{red!25} -18.5 & \cellcolor{red!10} -47.6 & \cellcolor{red!25} -42.7 \\ \cdashlinelr{1-4}
  \textbf{Permutation} & -5 & -28.5 & -11.9 \\
 \textbf{Trans. $\circ$ Perm.} & \cellcolor{red!25} -30.9 & \cellcolor{red!25} -62.6 & \cellcolor{red!25} -65.5 \\ \cdashlinelr{1-4}
  \textbf{Syntax} & -1.8 & -7.8 & -0.9 \\
 \textbf{Trans. $\circ$ Syntax} & \cellcolor{red!10} -7.2 & \cellcolor{red!10} -14.2 & \cellcolor{red!10} -3.5 \\  
\bottomrule
\end{tabular}
% Uncomment to resize resize
% }
\caption{\label{table:Composition:old}
Composing two transformations.
\zs{} is the zero-shot performance.
\supdiff~for a composed transformation is highlighted in \colorbox{red!25}{dark red} if it is much larger than the \supdiff~of individual transformations, and \colorbox{red!10}{light red} if it is comparable.
Trans=\textit{Transliteration}, Inv=\textit{Inversion}, Perm=\textit{Permutation}, Fr syntax=Change English corpus syntax to French corpus syntax.
Composing transformations always hurts ZS performance (\zs) when compared to single transformations.
\todo{Possible remove the \supdiff{} score in the main table and move the current version to the appendix. Explicitly mention the drops next to the scores of composed transformations.}
}
\end{table}


% \begin{table}[t]
% \centering
% % Uncomment to resize
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cccccccc}\toprule
% % Header -------------------------------------

% \multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Transformation}} & \multicolumn{2}{c}{\textbf{XNLI}} & \multicolumn{2}{c}{\textbf{NER}} & \multicolumn{2}{c}{\textbf{POS}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%  &  & \zs & \supdiff & \zs & \supdiff & \zs & \supdiff \\ \midrule
% \multirow{3}{*}{\textbf{Double}} & Trans. $\circ$ Inv. & 55.7 & \cellcolor{red!25} -18.5 & 32.5 &\cellcolor{red!10} -47.6 & 52.2 &\cellcolor{red!25} -42.7 \\
%  & Trans. $\circ$ Perm. & 44 & \cellcolor{red!25} -30.9 & 17.1 & \cellcolor{red!25} -62.6 & 29.5 & \cellcolor{red!25} -65.5 \\
%  & Trans. $\circ$ Fr syntax & 69.8 & \cellcolor{red!10} -7.2 & 53.5 & \cellcolor{red!10} -26.7 & 91.5 & \cellcolor{red!10} -3.5 \\ \midrule
% \multirow{4}{*}{\textbf{Single}} & Trans. & 74.1 & -2.1 & 78 & -2.3 & 94.6 & -0.5 \\
%  & Inv. & 73.2 & -2.5 & 39.8 & -40.7 & 94.4 & -0.8 \\
%  & Perm. & 68.6 & -7.5 & 40.2 & -40 & 78.3 & -16.7 \\
%  & Fr Syntax & 74.1 & -1.8 & 61.1 & -19.2 & 92.9 & -2.1 \\
% \bottomrule
% \end{tabular}
% % Uncomment to resize resize
% }
% \caption{Composing two transformations. \supdiff~for a double transformation is highlighted in dark red if it is much larger than the \supdiff~of individual transformations, and light red if it is comparable. Trans=\textit{Transliteration}, Inv=\textit{Inversion}, Perm=\textit{Permutation}, Fr syntax=Change English corpus syntax to French corpus syntax. \karthik{Re-order the rows in this table to have pairwise comparisons between compositions and their single counterparts, and add dashed lines in between the pairs.}}
% \label{table:Composition}
% \end{table}





==> Tables/EnglishInversion.tex <==
\begin{table}[t]
\centering
% Uncomment to resize
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccc}\toprule
% Header -------------------------------------
\multirow{2}{*}{\textbf{Vocabulary}} & \multicolumn{2}{c}{\textbf{XNLI}} & \multicolumn{2}{c}{\textbf{NER}} & \multicolumn{2}{c}{\textbf{POS}} & \multicolumn{2}{c}{\textbf{XQuAD}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}

 & \zs & \supdiff & \zs & \supdiff & \zs & \supdiff & \zs & \supdiff \\ \midrule

% Template
% English & 73.2 & -2.5  & 11.5 & 68.6 & -7.5  & 2.7 & 61.2 & -13.7 & -0.8 & 74.1 & -2.1 & 40.8 & 33.5 & -41   & 0 \\

\textbf{40000} & 73.5 & \ApplyGradient{-1.3} & 35.6 & \ApplyGradient{-43.8} & 94.6 & \ApplyGradient{-0.3} & 28.7 & \ApplyGradient{-44.3} \\
\textbf{20000} & 65.7 & \ApplyGradient{-9.9} & 40.3 & \ApplyGradient{-38.8} & 91 & \ApplyGradient{-3.7} & 34.9 & \ApplyGradient{-40} \\
\textbf{10000} & 63.5 & \ApplyGradient{-10.5} & 40.8 & \ApplyGradient{-35.2} & 69.1 & \ApplyGradient{-25.6} & 41.1 & \ApplyGradient{-29.5} \\

\bottomrule
\end{tabular}
% Uncomment to resize resize
}
\caption{Results for different vocabulary sizes and \textit{Inversion} transformation on English.}
\label{table:EnglishInversion}
\end{table}



==> Tables/HindiTransliterated.tex <==
\begin{table}
\centering
% \resizebox{1\columnwidth}{!}{
\begin{tabular}{c c c c}
\toprule

\textbf{Model} & \textbf{XNLI} & \textbf{NER} & \textbf{POS} \\ \midrule
\textbf{En-Hi} & 39 & 25 & 28.8 \\
\textbf{En-Trans(Hi)} & \textbf{60.6} & \textbf{57.4} & \textbf{62.5} \\

\bottomrule
\end{tabular}
% }
\caption{
Hindi transliteration
}
\label{table:hindi}
\end{table}
